PaaF: Raising the perceived quality of INR-Based Image Compression

Implicit Neural Representations (INRs) have recently emerged as a promising paradigm for image compression, offering a fundamentally different approach from traditional and learned codecs. Nevertheless, INR-based methods for image compression suffer from long encoding times and a consistent performance gap in classic quality metrics such as PSNR. In this work, we explore the potential of purely INR-based compression methods and we propose PaaF (Picture as a Function), a novel INR-based image codec that introduces improved architectural design, adaptive quantization, and an efficient entropy coding scheme. These components are designed to enhance rate-distortion performance while preserving the simplicity and parallelizability of INR-based decoding. Experimental results demonstrate consistent improvements over existing INR-based methods in both quantitative metrics and perceptual quality. These findings highlight the potential of INR-based approaches and contribute to narrowing the gap between functional representations and more established compression paradigms.

==> caption_formats.tex <==
\DeclareCaptionFormat{notsotiny}
{%
    \fontsize{6.00}{4}\selectfont #3
}

\DeclareCaptionFormat{tinytiny}
{%
    \fontsize{5.0}{4}\selectfont #3
}

\DeclareCaptionFormat{tiny}
{%
    \fontsize{4}{4}\selectfont #3
}

\DeclareCaptionFormat{cropfig}
{%
    \fontsize{5.25}{4}\selectfont #3
}

\DeclareCaptionFormat{cliccropfig}
{%
    \fontsize{3.0}{3.0}\selectfont #3
}

\newcommand{\preset}[1]{
    ``\textit{#1}''
}
